Investigating Retrieval Method Selection with Axiomatic Features

We consider algorithm selection in the context of ad-hoc information retrieval. Given a query and a pair of retrieval methods, we propose a meta-learner that predicts how to combine the methods' relevance scores into an overall relevance score. Inspired by neural models' different properties with regard to IR axioms, these predictions are based on features that quantify axiom-related properties of the query and its top ranked documents. We conduct an evaluation on TREC Web Track data and find that the meta-learner often significantly improves over the individual methods. Finally, we conduct feature and query weight analyses to investigate the meta-learner's behavior.

==> Makefile <==
###########################################################
#
# Makefile for LaTeX docs
#
# $Id: 
#

.SUFFIXES:
.SUFFIXES: .ps .dvi .tex

TEXINPUTS := .:${TEXINPUTS}
BIBINPUTS := .:${TEXINPUTS}

#all: eps dvi ps pdf # res
all: pdf
eps: fig obj

PAPER=main

LATEX=pdflatex

ps:  $(PAPER).ps

pdf: $(PAPER).pdf
dvi: $(PAPER).dvi

obj: $(patsubst %.obj, %.eps, $(wildcard *.obj))
fig: $(patsubst %.fig, %.eps, $(wildcard *.fig))

res:
	make -C results
	make -C figs

clean:
	$(RM) *.aux *.log *.bbl *.blg *~ \#*\# *.toc *.idx
	$(RM) $(patsubst %.tex, %.ps, $(wildcard *.tex))
	$(RM) $(patsubst %.tex, %.dvi, $(wildcard *.tex))
	$(RM) $(patsubst %.tex, %.pdf, $(wildcard *.tex))

distclean: clean
	$(RM) $(patsubst %.fig, %.eps, $(wildcard *.fig))
	$(RM) $(patsubst %.obj, %.eps, $(wildcard *.obj))

%.pdf: $(wildcard *.tex) $(wildcard *.bib)
	$(LATEX) $*
	bibtex $*
	$(LATEX) $*
	if [ -e $*.toc ] ; then $(LATEX) $* ; fi
	if [ -e $*.bbl ] ; then $(LATEX) $* ; fi
	if egrep Rerun $*.log ; then $(LATEX) $* ; fi
	if egrep Rerun $*.log ; then $(LATEX) $* ; fi
	if egrep Rerun $*.log ; then $(LATEX) $* ; fi

%.ps: %.dvi
	dvips -Ppdf -G0 -tletter -o $@ $<
%.ps.gz: %.ps
	gzip -v9 $<

%.eps: %.obj
	tgif -print -eps $*

%.eps: %.fig
	fig2dev -L eps $< $@


==> foo <==
\begin{thebibliography}{10}
\providecommand{\url}[1]{\texttt{#1}}
\providecommand{\urlprefix}{URL }
\providecommand{\doi}[1]{https://doi.org/#1}

\bibitem{cao2006RSVM}
Cao, Y., Xu, J., Liu, T.Y., Li, H., Huang, Y., Hon, H.W.: Adapting ranking svm
  to document retrieval. In: SIGIR'06 (2006)

\bibitem{recommender1}
Collins, A., Tkaczyk, D., Beel, J.: One-at-a-time: A meta-learning
  recommender-system for recommendation-algorithm selection on micro level.
  arXiv preprint arXiv:1805.12118  (2018)

\bibitem{townsend2006coh}
Cronen-Townsend, S., Zhou, Y., Croft, W.: Precision prediction based on ranked
  list coherence. In: Inf Retrieval'06 (2006)

\bibitem{dai2018convknrm}
Dai, Z., Xiong, C., Callan, J., Liu, Z.: Convolutional neural networks for
  soft-matching n-grams in ad-hoc search. In: AAAI'19 (2019)

\bibitem{federatedsearch2}
Demeester, T., Nguyen, D., Trieschnigg, D., Develder, C., Hiemstra, D.:
  Snippet-based relevance predictions for federated web search. In: Proceedings
  of the 35th European Conference on Information Retrieval Research. ECIR '13
  (2013)

\bibitem{fang2011axiom}
Fang, H., Tao, T., Zhai, C.: Diagnostic evaluation of information retrieval
  models. In: TOIS'11 (2011)

\bibitem{DRMM}
Guo, J., Fan, Y., Ai, Q., Croft, W.B.: A deep relevance matching model for
  ad-hoc retrieval. In: Proceedings of the 25th ACM International on Conference
  on Information and Knowledge Management. CIKM '16 (2016)

\bibitem{hauff2009survey}
Hauff, C., Azzopardi, L., Hiemstra, D.: The combination and evaluation of query
  performance prediction methods. In: ECIR'09 (2009)

\bibitem{he2006qpp}
He, B., Ounis, I.: Query performance prediction. In: Information Systems'06
  (2006)

\bibitem{he2003trec}
He, D., Demner-Fushman, D.: Hard experiment at maryland: From need negotiation
  to automated hard process. In: TREC'03 (2003)

\bibitem{he2008qc}
He, J., Larson, M., de~Rijke, M.: Using coherence-based measures to predict
  query difficulty. In: ECIR'08 (2008)

\bibitem{hui2017pacrr}
Hui, K., Yates, A., Berberich, K., de~Melo, G.: {PACRR}: A position-aware
  neural ir model for relevance matching. In: EMNLP'17 (2017)

\bibitem{copacrr}
Hui, K., Yates, A., Berberich, K., de~Melo, G.: Co-pacrr: A context-aware
  neural ir model for ad-hoc retrieval. In: WSDM 2018: The Eleventh ACM
  International Conference on Web Search and Data Mining (2018)

\bibitem{kingma2014adam}
Kingma, D., Ba, J.: Adam: A method for stochastic optimization. arXiv preprint
  arXiv:1412.6980  (2014)

\bibitem{bm25long}
Lv, Y., Zhai, C.: When documents are very long, bm25 fails! In: Proceedings of
  the 34th International ACM SIGIR Conference on Research and Development in
  Information Retrieval. SIGIR '11 (2011)

\bibitem{terrier}
Macdonald, C., McCreadie, R., Santos, R.L., Ounis, I.: From puppy to maturity:
  Experiences in developing terrier. Proc. of OSIR at SIGIR pp. 60--63 (2012)

\bibitem{mackenzie2018early}
Mackenzie, J., Culpepper, J., Blanco, R., Crane, M., Clarke, C.L., Lin, J.:
  Query driven algorithm selection in early stage retrieval. In: WSDM'18 (2018)

\bibitem{meltzer2007sdm}
Meltzer, D., W.B.C.: Latent concept expansion using markov random fields. In:
  SIGIR'07 (2007)

\bibitem{word2vec}
Mikolov, T., Sutskever, I., Chen, K., Corrado, G.S., Dean, J.: Distributed
  representations of words and phrases and their compositionality. In: Advances
  in neural information processing systems. pp. 3111--3119 (2013)

\bibitem{mothe2004ling}
Mothe, J., Tanguy, L.: Linguistic features to predict query difficulty. In:
  SIGIR Workshop on predicting Query Difficulty - Methods and Applications
  (2004)

\bibitem{nallapati2004feat}
Nallapati, R.: Discriminative models for information retrieval. In: SIGIR'04
  (2004)

\bibitem{nie2006sigir}
Nie, L., Davison, B.D., Qi, X.: Topical link analysis for web search. In:
  SIGIR'06 (2006)

\bibitem{qin2010Letor}
Qin, T., Liu, T.Y., Xu, J., Li, H.: Letor: A benchmark collection for research
  on learning to rank for information retrieval. In: Inf Retrieval'10 (2010)

\bibitem{renningsaxiomatic}
Rennings, D., Moraes, F., Hauff, C.: An axiomatic approach to diagnosing neural
  ir models  (2019)

\bibitem{bm25}
Robertson, S.E., Walker, S.: Some simple effective approximations to the
  2-poisson model for probabilistic weighted retrieval. In: Proceedings of the
  17th Annual International ACM SIGIR Conference on Research and Development in
  Information Retrieval. SIGIR '94 (1994)

\bibitem{mcdonald2018posit}
Ryan~McDonald, Georgios-Ioannis~Brokos, I.A.: Deep relevance ranking using
  enhanced document-query interactions. In: EMNLP'18 (2018)

\bibitem{Severyn15}
Severyn, A., Moschitti, A.: Learning to rank short text pairs with
  convolutional deep neural networks. In: Proceedings of the 38th International
  ACM SIGIR Conference on Research and Development in Information Retrieval.
  SIGIR '15 (2015)

\bibitem{federatedsearch}
Shokouhi, M., Si, L.: Federated search. vol.~5 (Jan 2011)

\bibitem{shtok2012dist}
Shtok, A., Kurland, O., Carmel, D., Raiber, F., Markovitis, G.: Predicting
  query performance by query-drift estimation. In: ACM Trans Inf. Syst.'12
  (2012)

\bibitem{tang2019dtb}
Tang, Z., Hui~Yang, G.: Deeptilebars: Visualizing term distribution for neural
  information retrieval. In: AAAI'19 (2019)

\bibitem{tao2007prox}
Tao~Tao, C.Z.: An exploration of proximity measures in information retrieval.
  In: SIGIR'07 (2007)

\bibitem{winavar2007lm}
Winaver, M., Kurland, O., Domshlak, C.: Towards robust query expansion: Model
  selection in the language modelling framework. In: SIGIR'07 (2007)

\bibitem{wu2002fusion}
Wu, S., Crestani, F.: Data fusion with estimated weights. In: CIKM'02 (2002)

\bibitem{xiong2017end}
Xiong, C., Dai, Z., Callan, J., Liu, Z., Power, R.: End-to-end neural ad-hoc
  ranking with kernel pooling. In: SIGIR'17

\bibitem{xu2005rank}
Xu, J., Cao, Y., Li, H., Zhao, M.: Ranking definitions with supervised learning
  methods. In: WWW'05 (2005)

\bibitem{tov2005meta}
Yom-Tov, E., Fine, S., Carmel, D., Darlow, A.: Learning to estimate query
  difficulty: Including applications to missing content detection and
  distributed information retrieval. In: SIGIR'05 (2005)

\bibitem{zammani2018neural}
Zammani, H., Croft, W., Culpepper, J.: Neural query performance prediction
  using weak supervision from multiple signals. In: SIGIR'18 (2018)

\bibitem{zhou2006robust}
Zhou, Y., Croft, W.: Ranking robustness: A novel framework to predict query
  performance. In: CIKM'06 (2006)

\bibitem{zhou2007web}
Zhou, Y., Croft, W.: Query performance prediction in web search. In: SIGIR'07
  (2007)

\end{thebibliography}

